DeformToon3D: Deformable 3D Toonification from Neural Radiance Fields

In this paper, we address the challenging problem of 3D toonification, which involves transferring the style of an artistic domain onto a target 3D face with stylized geometry and texture. Although fine-tuning a pre-trained 3D GAN on the artistic domain can produce reasonable performance, this strategy has limitations in the 3D domain. In particular, fine-tuning can deteriorate the original GAN latent space, which affects subsequent semantic editing, and requires independent optimization and storage for each new style, limiting flexibility and efficient deployment. To overcome these challenges, we propose DeformToon3D, an effective toonification framework tailored for hierarchical 3D GAN. Our approach decomposes 3D toonification into subproblems of geometry and texture stylization to better preserve the original latent space. Specifically, we devise a novel StyleField that predicts conditional 3D deformation to align a real-space NeRF to the style space for geometry stylization. Thanks to the StyleField formulation, which already handles geometry stylization well, texture stylization can be achieved conveniently via adaptive style mixing that injects information of the artistic domain into the decoder of the pre-trained 3D GAN. Due to the unique design, our method enables flexible style degree control and shape-texture-specific style swap. Furthermore, we achieve efficient training without any real-world 2D-3D training pairs but proxy samples synthesized from off-the-shelf 2D toonification models.

==> tabs_and_figs/fig_teaser.tex <==
% !TEX root = ../main.tex
\begin{figure*}[h!]
\begin{center}
  \includegraphics[width=1\linewidth]{figures/teaser.pdf}
\end{center}
  \caption{Teaser figure place holder. TODO include: toonification results, mulit style, multi view, surface; synthesis? Need to decide. Our method achieves multi-style toonification with a single model.}
\label{fig:teaser}
\end{figure*}
